Extended Labeled Faces in-the-Wild (ELFW): Augmenting Classes for Face Segmentation

Existing face datasets often lack sufficient representation of occluding objects, which can hinder recognition, but also supply meaningful information to understand the visual context. In this work, we introduce Extended Labeled Faces in-the-Wild (ELFW), a dataset supplementing with additional face-related categories -- and also additional faces -- the originally released semantic labels in the vastly used Labeled Faces in-the-Wild (LFW) dataset. Additionally, two object-based data augmentation techniques are deployed to synthetically enrich under-represented categories which, in benchmarking experiments, reveal that not only segmenting the augmented categories improves, but also the remaining ones benefit.

==> auxiliar_tex/miscellaneous.tex <==

\textcolor{red}{No tengo claro que se necesite este estado del arte en semantic segmentation. Tendría sentido si estuviéramos proponiendo una nueva manera de hacer semantic segmentation, pero nuestro foco es el dataset y dar unos números orientativos de cómo funciona el estado del arte en el mismo.}
\textcolor{green}{Tendría sentido para introducir DeepLab+v3, pero igualmente se podría reducir}

Probably, the first remarkable work on semantic segmentation by means of Fully Convolutional Networks (FCN) was performed by Long et al.~\cite{long2015fully}. Following works have been essentially facing a challenging problem associated with the intrinsic nature of deep neural networks, which consists on how to recover the spatial information compacted in the latent space at the very last neural layers. Most of the works deal with it by stacking upsampling layers at the network's output until the predicted labels are pixel-wise, so input and output are the same size. Thus, terms such as upconvolution, unpooling, deconvolution, atrous deconvolution, dilated convolution, and even stride transpose convolution have been used to refer to the same concept with different variations and performances~\cite{yu2015multi, noh2015learning, chen2017deeplab}. A second significant strategy, often used in combination, consists on preserving the residual spatial information at each pooling level to be later aggregated into each unpooling level. This can be seen as a particular type of Residual Neural Network (RNN) arranged in form of a multi-scale or multi-resolution architecture~\cite{ronneberger2015u, yu2015multi, ghiasi2016laplacian, peng2017large, pohlen2017full, zhao2017pyramid, lin2017refinenet, yang2018denseaspp}. Furthermore, some works take advantage of Conditional Random Fields (CRF), a structure prediction model and the state of the art in the pre-deep learning era, which may help to refine spatially incoherent areas, especially regarding their compactness and contour irregularities. CRFs have been equally used as a posterior processing stage~\cite{noh2015learning}, but also inherently in the formulation of the network architecture itself~\cite{chen2014semantic, zheng2015conditional, liu2015multi, chandra2016fast, saito2016real}. Additionally, recent works propose to use lately popular attention networks~\cite{fu2019dual}.








\section{Metrics}

Vamos a entender las métricas del paper de la FCN:
\begin{itemize}
    \item $n_{ij}$ es el número de píxeles de la clase $i$ predecidos cómo de la clase $j$.
    \item $n_{\text{cl}}$ el número de clases
    \item $t_i = \sum_{j}n_{ij}$ el número de píxeles totales de la clase $i$.
\end{itemize}
Primeras observaciones:
$$
t_i = n_{ii} + \sum_{j \neq i} n_{ij} = TP_i + FN_i
$$
es decir, $t_i$ son todos los píxeles de la clase $i$ (ya lo dice en la definición), pero aquí los dividimos entre todos los píxeles que se han acertado ($TP_i$) y los que se han clasificado cómo otra clase ($FN_i$). 

\begin{enumerate}

\item \textbf{Pixel accuracy}: $\frac{\sum_{i} n_{ii}}{\sum_{i}t_i}$

Arriba tenemos todos los pixeles que se han acertado de todas las clases. O todos los $TP$ de todas las clases. O lo que en el código es $(predictions==labels).sum()$.

Abajo tenemos todos los píxeles de la imagen, porque es la suma de todos los píxeles de todas las clases.

Por lo tanto, esta medida es la que veníamos calculando con el nombre $val\_acc$.

Este valor no podemos calcularlo por separado para cada clase. Su versión por clase seria lo siguiente:

\item \textbf{Mean accuracy}: $\frac{1}{n_{\text{cl}}} \sum_{i} \frac{n_{ii}}{t_i}$

Si reescribimos, esto es  $\frac{n_{ii}}{t_i} = \frac{TP_i}{TP_i+FN_i}$, por lo tanto el $TPR$ de la clase $i$ ($TPR_i$). Por lo tanto, este \textit{mean accuracy} es la media para todas las clases de lo que nosotros llamábamos true positive rate o recall.  

Podemos calcularlo por separado para cada clase y luego sacar su media.

\item \textbf{Mean IU}: $\frac{1}{n_{\text{cl}}} \sum_{i} \frac{n_{ii}}{t_i + \sum_{j}n_{ji} - n_{ii}}$

Ojo aquí: $\sum_{j}n_{ji}$ son todos los píxeles de todas las clases predecidas como de la clase $i$. O sea, $\sum_{j}n_{ji} = n_{ii} + \sum_{j \neq i} n_{ji}$ que son los $TP$ de la clase $i$ ($TP_i$) y los $FP$ de la clase $i$ ($FP_i$). 

Reescribiendo, tenemos:

$$ \frac{n_{ii}}{t_i + \sum_{j}n_{ji} - n_{ii}} = $$
$$ = \frac{TP_i}{(TP_i + FN_i) + (TP_i + FP_i) - TP_i} = $$
$$ = \frac{TP_i}{TP_i + FN_i + FP_i}$$

esto se llama Threat score (TS) or Critical Success Index (CSI) en 

{\small https://en.wikipedia.org/wiki/Sensitivity\_and\_specificity}

Se calcula para cada clase y se saca media para todas las clases.

\item \textbf{Frequency weighted IU}: lo mismo que antes pero normalizando de alguna manera en función de la aparición de cada clase en la imagen.

$$ \frac{1}{\sum_{k}t_k} \sum_{i} \frac{t_i \cdot n_{ii}}{t_i + \sum_{j}n_{ji} - n_{ii}} = $$
$$ =\sum_{i} \frac{t_i }{\sum_{k}t_k} \cdot \frac{n_{ii}}{t_i + \sum_{j}n_{ji} - n_{ii}} = $$
$$ \sum_{i} \frac{t_i }{\sum_{k}t_k} \cdot TS_i = \sum_{i} \omega_i \cdot TS_i $$
donde $\omega_i$ está pesando la contribución de la clase en la imagen, ya que $t_i$ son los píxeles de la clase $i$ y $\sum_k t_k$ son todos los píxeles de la imagen. $TS_i$ es la medida del punto anterior para la clase $i$.
\end{enumerate}



\iffalse
During the last decade, deep learning has taken the state-of-the-art performance in most computer vision challenges, and semantic segmentation is not an exception. Probably, the first remarkable work on semantic segmentation by means of Fully Convolutional Networks (FCN) was performed by Long et al.~\cite{long2015fully}. The subsequent works have been essentially facing how to recover at the very last neural layers the spatial information compacted in the latent space, a challenging problem associated with the intrinsic nature of deep neural networks. Most of the works deal with it by stacking upsampling layers\footnote{Upconvolution, unpooling, deconvolution, atrous deconvolution, dilated convolution, and even stride transpose convolution have been used to refer to the same concept with different variations and performances.}  
%~\cite{yu2015multi, noh2015learning, chen2017deeplab
until the predicted labels are pixel-wise, and also by preserving the residual spatial information at each pooling level to be later aggregated into each unpooling level (multi-scale approaches); being DeepLabV3~\cite{chen2017deeplab} among the most referenced state-of-the-art multi-scale upconvolution architectures.

In this section, it is assessed how the proposed ELFW dataset, with extending and augmented categories, can be efficiently learned by FCN on semantic segmentation. Hence, we are not interested in comparing multiple neural architectures, not even a tough training optimization. With this in mind, we opted for these two architectures previously mentioned, i.e. the so to speak `vanilla' FCN and DeepLabV3. These elections were also motivated by the non-negligible reason of having officially released implementations.
\fi



{\color{blue}
Global Convolutional Network (GCN)~\cite{peng2017large}
Among the SoTA architectures, these are the most relevant CNN with available code.

Fully Convolutional Network (FCN)
Global Convolutional Network (GCN-ZijunDeng, GCN-ycszen)
Dual Attention Network (DANET)
Although the original DANET code was released by the authors, several conflicts with package version made the code impractical. Here we list some troubleshouting issues found during the process of making it work.

The GCN architecture proposes a multi-scale approach made of a 4-layered Resnet152 combined with several GCN and Boundary Refinement modules for each level. All levels are upsampled (deconvolved) and summed up to the original resolution afterwards. This net has been proposed in:


Since authors did not release the code, both implementations GCN-ZijunDeng and GCN-ycszen are a well trade-off between the original architecture and a documented Pytorch code. However the former originally released by ZijunDeng uses independent losses for each scale together with other architecture discrepancies which does not strictly follow the guidelines suggested in the original publication. We finally leaned for the latter candidate released by ycszen. Although this code does not implement the Restnet-GCN module originally proposed in the paper.
}



{\color{blue}
The original paper [0] Fully Convolutional Networks for Semantic Segmentation claims: (1) there's no evidence that Unnormalized Softmax where classes compete provides better results than Sigmoid Cross Entropy Loss. (2) No evidence class balancing improves results. (3) Increasing batch-size over iterations helped to train.

Because the original LFW image resolution is smaller than the size of the dataset originally used in the GCN paper, the number of multi-scale levels were reduced from 4 to 3 and the kernel size from 11 to 7 during the initial trials.
Also Resnet50 instead of Resnet152 was used to alleviate computation and training convergence.

Data augmentation (scaling, shifting, and horizontal flips) has been used for all the experiments showed here. Note it must be avoided at first to validate overfitting on a reduced training set.

Xavier initialization instead of kaiming seemed to make the difference for the model to converge.

GCN 3 multiscale levels delivered better results than both 4 and 2 levels for the first dataset. The former has a too coarse resolution, 8x8 for input images of 250x250, and the latter delivered noisier results probably due to too short filters to detect broad features across the image. Also 2 levels seemed to have more difficulties to converge when the dataset is increased with more categories and images.

Although the validation loss gets exhausted, for instance symptoms of overfitting appear beyond 100 epochs with 3 levels, the validation accuracy reveals that there is still more room for the net to learn and improve results beyond those 100 epochs.

For that reason early stop on accuracy was used for all experiments, ranging from 60 to 100 epochs without validation accuracy improvement.
The learning rate however must depend exclusively on the training set. Although it was scheduled with 10 epoch patience, the initial lr=10-4 behave adequately and constant during the all the training tests since the training loss decreased nicely and smoothly.

On the contrary, if the dataset is augmented with more images, the 4 levels architecture seems to preform slightly better. On webcam experiments some errors could be noticed for instance to handle the extra mouth-mask category by using 3 levels. From this one could argue that in principle the more levels the net has the more knowledge it can acquire.

Two common mistakes made by the GCN net is to mis-classify regular glasses as sunglasses and hair as wearable when a wearable is actually put on. The way the ELFW was labeled has probably much to do with it.

The sunglasses category improved around 15\% points after training with the artificially augmented dataset and in general all the categories showed an overall improvements. Note than the augmented dataset contains more than 50\% of images than the basic dataset, and the augmented+occluded contains more than 110\% of images. Therefore at each epoch the amount of newly feed images is considerably higher.

The above means that the model is able to acquire even more knowledge than initially expected. And therefore it's reasonable to think that extending the current dataset with even more images could probably increase the current results.

The simplest GCN model and the basic dataset converged in around 2 hours, while the complexest and augmented+occluded dataset converged in more than 20 hours with a GeForce GTX 970.
}


\iffalse
\begin{itemize}
    \item Pixel Accuracy: a class-independent global measure consisting in the ratio between the all true positives (TP) and all pixels across the image or batch.
    \item Mean Accuracy: averages the True Positive Ratio for all classes $\sum_i{TPR_i}=\sum_i{\frac{TP_i}{TP_i+FN_i}}$ where only false negatives $F$ intervene as negative factor.
    \item Mean IU: is the averaged ratio across classes between the intersection of the predicted and ground-truth areas and its union, also named the averaged Threat Score or Critical Success Index. It can be formulated as $\sum_i{TS_i}=\sum_i{\frac{TP_i}{TP_i+FN_i+FP_i}}$, which takes into account also false positives (FP) or the misclassified pixels originally labeled with a different class. The frequently reported F1-Score behaves similarly on account of a mere different correction factor, and so it's not included in this study.
    \item Frequency Weighted IU: is the averaged ratio $TS$ across classes weighted according to the normalized class appearance frequency.
\end{itemize}
\fi

Subsequent works have been essentially facing how to recover at the very last neural layers the spatial information compacted in the latent space. Most of them deal with it by stacking upsampling layers until the predicted labels are pixel-wise, and also by preserving the residual spatial information at each pooling level to be later aggregated into each unpooling level (multi-scale approaches);

==> auxiliar_tex/propuesta_jaume.tex <==
% ----------------------------------------------------------------------

\section{Experiments: facial semantic segmentation - \textcolor{red}{Propuesta Jaume hasta ``Validation tests''}}

In this section we provide benchmarking results by using the ELFW dataset on semantic segmentation, a natural framework for the released type of data. We used two deep neural networks of the semantic segmentation state of the art. In particular, we used the Fully Convolutional Network (FCN) originally proposed in the seminal work~\cite{long2015fully} and a much recent architecture such as DeepLabV3~\cite{chen2017deeplab} which has been reported to perform remarkably well in several standard datasets.


\subsection{Baseline configuration}

\noindent\textbf{Training hyper-parameters}: 
To provide a common baseline for the chosen architectures from which establish results on ELFW, all experiments here conducted were configured alike. We used a COCO train2017 pre-trained ResNet-101 backbone for both FCN and DeepLabV3. Then, fine-tuning was performed by minimizing a \textcolor{blue}{pixel-wise cross entropy loss} under a $16$ batch sized SGD optimizer using a multi-step learning rate scheduled to provoke an initial fast learning with $10^{-3}$ at the very first epochs, to be latter lowered to $2^{-4}$ and then $0.4^{-5}$ at epochs $35$ and $90$, respectively, where performance stabilized. Weight decay was set to $5^{-4}$ and momentum to $0.99$. In all experiments basic data augmentation such as random horizontal flips, affine shifts and image resize transformations were used. Training was set to go off after 30 epochs without improving.

\medskip\noindent\textbf{Augmentation factor}: 
In order to evaluate the proposed category augmentation strategies we defined $\sigma$ to be the factor denoting the number of assets-based augmentation faces added to the baseline training dataset. For instance, $\sigma=0.5$ means that an extra $50\%$ with respect to the baseline train set size ($3,754$) of synthetically augmented images have been added for training, \ie $1,877$ augmented images. \textcolor{blue}{When more than one augmentation asset is used for augmentation, this factor is distributed uniformly among the different types.}

\medskip\noindent\textbf{Validation sets}: 
To assess each of the augmented categories separately and jointly, we defined different validation sets related to the nature of each augmented data.
The size of each validation set was set to a $10\%$ of the ELFW dataset, $376$ images in total. When augmenting sunglasses, the validation set contained $50\%$ of the images originally wearing real sunglasses within the whole dataset, which was found to be $62$ out of $125$ in total ---the other half is reserved for the training split---. The rest of the validation set is randomly populated with the remaining faces in the ELFW dataset. Likewise, the hand augmentation validation set contained $28$ faces originally occluded by real hands, from the $56$ found in total. Finally, when training with both augmentation types or even with mouth-masks, an unconstrained random set was constructed regardless of sunglasses or hands.

\medskip\noindent\textbf{Hardware and software}: 
Each of the neural models was trained on an individual Nvidia GTX 1080Ti GPU. Independently of the network architecture, the configuration with the smallest dataset ($\sigma=0$) required about $1$ day of training, while that with the largest one ($\sigma=1$) took about a week. 
We used the Pytorch $1.1.0$ and torchvision $0.3.0.$ versions which officially released code for the FCN and DeeplabV3 models\footnote{Pytorch models~\href{ https://pytorch.org/docs/stable/torchvision/models.html}{https://pytorch.org/docs/stable/torchvision/models.html}} that come with the pre-trained backbones mentioned above.

==> auxiliar_tex/todo_notes.tex <==

\textcolor{blue}{Aquí va mi propuesta para esta sección (para acordarme de lo que pienso a día 18.12.2019)}:
\begin{itemize}

    \item Un primer párrafo de introducción diciendo que aquí lo que se quiere es establecer un baseline y que tomamos dos arquitecturas del estado del arte. Que además nos sirven para validar el data augmentation.
    
    \item Subsección: \textbf{implementation details} hablar de que usamos los modelos preentrenados (en un subset de COCO train2017 para 20 clases\footnote{\href{https://pytorch.org/docs/stable/torchvision/models.html\#semantic-segmentation}{https://pytorch.org/docs/stable/torchvision/models.html\#semantic-segmentation}}) de pytorch (podemos incluso mencionar la versión de torchvision que usamos) y muy brevemente decir los parámetros que se han usado (hasta cuando se ha entrenado, etc.), sin necesidades de entrar en muchos detalles porqué el objetivo no es petar los resultados si no mostrar un baseline. Resnet 101.
    
    \item Subsección: \textbf{Category augmentation} hablar de las métricas que se usan, los validation sets para cada caso, la manera de aumentar los datasets (definir los ratios $\sigma$), mostrar los resultados (en tablas o curvas) y, finalmente, comentarlos. De nuevo, el objetivo no es petarlo y hay que hacer comentarios generales sobre la metodologia y ponerlo en contexto de otros métodos similares.\textcolor{blue}{Incluir resultados gráficos de cómo mejoran las gafas con $\sigma$ y también otras clases al aumentar con manos.}
    
    \item Subsección: \textbf{Qualitative results} aquí mostramos cosas como ``extending labels in the lab'' y aparte de comentar los resultados (lo que ya está más o menos escrito), hay que hacer hincapié en que el modelo puede generalizar con classes de las que nunca ha visto casos reales (las máscaras), y aunque aquí no pueden darse números porqué no hay groundtruth, esto debería ser un buen punto. En esta sección usamos el modelo entrenado con todas las clases (incluídas las máscaras).

    % \item Rellenar tablas
    % \item Resumir estado del arte SS.
    % \item Describir hyperparams y versiones software usadas.
    %\item Describir validation sets.    
    \item Generar ejemplos graficos de gafas y manos en funcion de epocas y aumentos.
    \item Generar ejemplos webcam.
    
    \item enfoque biometrics
    \item conclusions y abstract
    
\end{itemize}
